Redshift-space distortions in simulations of the 21-cm signal from the cosmic dawn

The 21-cm signal from the Cosmic Dawn (CD) is likely to contain large fluctuations, with the most extreme astrophysical models on the verge of being ruled out by observations from radio interferometers. It is therefore vital that we understand not only the astrophysical processes governing this signal, but also other inherent processes impacting the signal itself, and in particular line-of-sight effects. Using our suite of fully numerical radiative transfer simulations, we investigate the impact on the redshifted 21-cm from the CD from one of these processes, namely the redshift-space distortions (RSDs). When RSDs are added, the resulting boost to the power spectra makes the signal more detectable for our models at all redshifts, further strengthening hopes that a power spectra measurement of the CD will be possible. RSDs lead to anisotropy in the signal at the beginning and end of the CD, but not while X-ray heating is underway. The inclusion of RSDs, however, decreases detectability of the non-Gaussianity of fluctuations from inhomogeneous X-ray heating measured by the skewness and kurtosis. On the other hand, mock observations created from all our simulations that include telescope noise corresponding to 1000 h observation with the Square Kilometre Array telescope show that we may be able image the CD for all heating models considered and suggest RSDs dramatically boost fluctuations coming from the inhomogeneous Ly-$\alpha$ background.

==> defn.tex <==

\def\aj{AJ}% % Astronomical Journal
\def\an{Astron. Nachr.}% % Astronomical Nachr.
\def\ab{Astrophysical Bulletin}% % Astronomical Nachr.
%\def\actaa{Acta Astron.}% % Acta Astronomica
\def\araa{ARA\&A}% % Annual Review of Astron and Astrophys
\def\apj{ApJ}% % Astrophysical Journal
\def\apjl{ApJL}% % Astrophysical Journal, Letters
\def\apjs{ApJS}% % Astrophysical Journal, Supplement
\def\ao{Appl.~Opt.}% % Applied Optics
\def\apss{Ap\&SS}% % Astrophysics and Space Science
\def\aap{A\&A}% % Astronomy and Astrophysics
\def\aapr{A\&A~Rev.}% % Astronomy and Astrophysics Reviews
\def\aaps{A\&AS}% % Astronomy and Astrophysics, Supplement
\def\azh{AZh}% % Astronomicheskii Zhurnal
\def\baas{BAAS}% % Bulletin of the AAS
\def\bac{Bull. astr. Inst. Czechosl.}% Bulletin of the Astronomical vakia
\def\basi{Bull. Astron. Soc. India}% Bulletin of the Astronomical Soc. India  
\def\caa{Chinese Astron. Astrophys.}% % Chinese Astronomy and Astrophysics
\def\cbet{Cent. Bur. Electron. Telegrams}% Central Buareu Electronic Telegrams
\def\cjaa{Chinese J. Astron. Astrophys.}% % Chinese Journal of Astronomy  
\def\icarus{Icarus}% % Icarus
\def\jcap{J. Cosmology Astropart. Phys.}% % Journal of Cosmology and Asics
\def\jrasc{J. R. Astron. Soc. Canada}% % Journal of the RAS of Canada
\def\mnras{MNRAS}% % Monthly Notices of the RAS
\def\memras{MmRAS}% % Memoirs of the RAS
\def\na{New A}% % New Astronomy
\def\nar{New A Rev.}% % New Astronomy Review
\def\pasa{PASA}% % Publications of the Astron. Soc. of Australia
\def\pra{Phys.~Rev.~A}% % Physical Review A: General Physics
\def\prb{Phys.~Rev.~B}% % Physical Review B: Solid State
\def\prc{Phys.~Rev.~C}% % Physical Review C
\def\prd{Phys.~Rev.~D}% % Physical Review D
\def\pre{Phys.~Rev.~E}% % Physical Review E
\def\prl{Phys.~Rev.~Lett.}% % Physical Review Letters
\def\pasp{PASP}% % Publications of the ASP
\def\pasj{PASJ}% % Publications of the ASJ
\def\qjras{QJRAS}% % Quarterly Journal of the RAS
\def\rmxaa{Rev. Mexicana Astron. Astrofis.}% % Revista Mexicana de Astronomia  
\def\rmxaac{Rev. Mexicana Astron. Astrofis. Ser. Conf.}% % Revista Mexicana de Astronomia  
\def\sci{Science}% % Science  
\def\skytel{S\&T}% % Sky and Telescope
\def\solphys{Sol.~Phys.}% % Solar Physics
\def\sva{Sov.~Astron.}% % Soviet Astronomy
\def\sovast{Sov.~Astron.}% % Soviet Astronomy
\def\sval{Sov.~Astron.~Lett.}% % Soviet Astronomy Letters
\def\ssr{Space~Sci.~Rev.}% % Space Science Reviews
\def\zap{ZAp}% % Zeitschrift fuer Astrophysik
\def\nat{Nature}% % Nature
\def\iaucirc{IAU~Circ.}% % IAU Cirulars
\def\aplett{Astrophys.~Lett.}% % Astrophysics Letters
\def\apspr{Astrophys.~Space~Phys.~Res.}% % Astrophysics Space Physics Research
\def\bain{Bull.~Astron.~Inst.~Netherlands}% % Bulletin Astronomical erlands
\def\fcp{Fund.~Cosmic~Phys.}% % Fundamental Cosmic Physics
\def\gca{Geochim.~Cosmochim.~Acta}% % Geochimica Cosmochimica Acta
\def\grl{Geophys.~Res.~Lett.}% % Geophysics Research Letters
\def\jcp{J.~Chem.~Phys.}% % Journal of Chemical Physics
\def\jgr{J.~Geophys.~Res.}% % Journal of Geophysics Research
\def\jqsrt{J.~Quant.~Spec.~Radiat.~Transf.}% % Journal of Quantitiative r
\def\memsai{Mem.~Soc.~Astron.~Italiana}% % Mem. Societa Astronomica Italiana
\def\nphysa{Nucl.~Phys.~A}% % Nuclear Physics A
\def\physrep{Phys.~Rep.}% % Physics Reports
\def\physscr{Phys.~Scr}% % Physica Scripta
\def\planss{Planet.~Space~Sci.}% % Planetary Space Science
\def\procspie{Proc.~SPIE}% % Proceedings of the SPIE


